Aligning Misaligned Benchmarks for Single-View Novel View Synthesis

While single-view novel view synthesis methods have been dramatically enhanced recently, how to quantify their performance has yet to be standardized. In this work, we demonstrate that an important factor lies in how each method's own reference frame is aligned with the so-called ground-truth pose. Existing methods often rely on test-time optimization of target poses for this alignment, which inherently is ill-posed due to the complexity of the optimization landscape of camera poses vs render accuracy, leading to methods being evaluated at an arbitrary local optimum. Some recognize this limitation and thus rely on 3D reconstructions of entire scenes using training and test views to align poses, which may be infeasible. In this work, instead, we propose to use traditional 2D-to-2D and 2D-to-3D image matching techniques to align 3D reconstructions. We also evaluate only within co-visible regions, between different views, which is the only place where a `correct' ground truth can be defined. Our evaluations show that with proper coordinate alignment, novel-view synthesis methods that use explicit 3D Gaussians achieve the state of the art, despite being previously reported in the literature to be outperformed by pure image-based 2D methods. We further provide a simple baseline that directly utilizes an off-the-shelf video generator and a feed-forward geometry estimator. Our simple baseline is already comparable to state-of-the-art methods specifically trained for novel-view synthesis, without any task-specific training.

==> Makefile <==
# Makefile for the WACV 2027 paper.
#
#   make            build main.pdf (latexmk: runs pdflatex/bibtex + reruns as needed)
#   make watch      continuous preview build, recompiles on every save
#   make view       build, then open the PDF (macOS `open`)
#   make manual     build without latexmk (explicit pdflatex/bibtex passes)
#   make clean      remove build artifacts, keep the PDF
#   make cleanall   remove build artifacts and the PDF

MAIN    := main
FLAGS   := -pdf -interaction=nonstopmode -halt-on-error -file-line-error

.PHONY: all watch view manual clean cleanall

# Default: latexmk decides what needs rebuilding (via its own .fls/.fdb tracking)
# and runs bibtex automatically, so it is safe to always invoke.
all:
	latexmk $(FLAGS) $(MAIN).tex

watch:
	latexmk $(FLAGS) -pvc $(MAIN).tex

view: all
	open $(MAIN).pdf

# Fallback for environments without latexmk.
manual:
	pdflatex -interaction=nonstopmode -halt-on-error $(MAIN).tex
	bibtex $(MAIN)
	pdflatex -interaction=nonstopmode -halt-on-error $(MAIN).tex
	pdflatex -interaction=nonstopmode -halt-on-error $(MAIN).tex

clean:
	latexmk -c $(MAIN).tex 2>/dev/null || \
	  rm -f $(MAIN).aux $(MAIN).bbl $(MAIN).blg $(MAIN).log $(MAIN).out \
	        $(MAIN).brf $(MAIN).fls $(MAIN).fdb_latexmk $(MAIN).synctex.gz

cleanall:
	latexmk -C $(MAIN).tex 2>/dev/null || \
	  rm -f $(MAIN).aux $(MAIN).bbl $(MAIN).blg $(MAIN).log $(MAIN).out \
	        $(MAIN).brf $(MAIN).fls $(MAIN).fdb_latexmk $(MAIN).synctex.gz $(MAIN).pdf


==> figures/eval_overview/item.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/eval_overview/eval_overview}
    \caption{
        {\bf Evaluation protocol overview --}
        \ky{%
        We find the camera that best renders the test view by starting from a `best-effort' rendering of this view, and then performing a 2D-to-2D matching between the rendered view and the test view. 
        We then use 2D-to-3D correspondences of the rendered view, which we obtain with the reconstructed 3D model.
        With these two correspondences, we then estimate the camera pose using a Perspective-n-Point (PnP) algorithm.
        We further refine the camera pose via conventional test-time optimization, but only on the co-visible regions and computed evaluation metrics within this region.
        }%
    }
    \label{fig:eval_overview}
\end{figure}




==> figures/nvs_overview/item.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/nvs_overview/nvs_overview}
    \caption{
        {\bf Novel-view synthesis overview --}
        \TODO{caption}
    }
    \label{fig:nvs_overview}
\end{figure}




==> figures/viewpoint_separation/item.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/viewpoint_separation/viewpoint_separation.pdf}
    \caption{\yt{\textbf{Input--target viewpoint separation.}
    Rotation-geodesic angle between the input view and each target view, over all $1678$ evaluation pairs
    (box: quartiles, whiskers: $10$--$90$th percentile, dots: individual pairs).
    Every dataset except \dlthreedv\ uses the benchmark-provided input view, so these are the separations induced by existing protocols;
    for \dlthreedv\ we show our re-balanced split, whose input view is chosen to maximize co-visibility with the remaining cameras rather than to minimize viewpoint change---its angular separations remain comparable to the original benchmark input view (median $39.2^\circ$ vs.\ $39.7^\circ$).
    Medians range from $5^\circ$ (\retenk) to $39^\circ$ (\dlthreedv), and the tail is long:
    $16\%$ of all pairs exceed $45^\circ$ and $17\%$ of \dlthreedv\ pairs exceed $90^\circ$, reaching $179^\circ$.
    Beyond $90^\circ$ the two views hardly co-observe the scene, making the comparison largely uninformative.}}
    \label{fig:viewpoint_separation}
\end{figure}

